The ($\Gamma$-asymptotic) wavefront sets: $GL_n$

Let $G$ be a connected reductive $p$-adic group. As verified for unipotent representations, it is expected that there is a close relation between the (Harish-Chandra-Howe) wavefronts sets of irreducible smooth representations and their Langlands parameters in the local Langlands correspondence via the Lusztig-Spaltenstein duality and the Aubert-Zelevinsky duality. In this paper, we define the $\Gamma$-asymptotic wavefront sets generalizing the notion of wavefront sets via the $\Gamma$-asymptotic expansions (in the sense of Kim-Murnaghan), and then study the their relation with the Langlands parameters. When $G=GL_n$, it turns out that this reduces to the corresponding relation of unipotent representations of the appropriate twisted Levi subgroups via Hecke algebra isomorphisms. For unipotent representations of $GL_n$, we also describe the Harish-Chandra-Howe (HCH) local character expansions of irreducible smooth representations using Kazhdan-Lusztig theory, and give another computation of the coefficients in the HCH expansion and the wavefront sets.

==> wave-prelim.tex <==



\subsection{\bf Basic notation and definitions}

\begin{numbering}
{\bf Notation.}\rm\ 
Let $F$ be a $p$-adic field with residue field $\bbF_q$ equipped with the norm $|\cdot|$.
Let bold face letters $\bG$, $\bH$ etc denote reductive groups over $F$, and corresponding roman letters the group of $F$-rational points. In particular, we let $\bG_n$ denote $\bGL_n$. Similarly, $\blieG$, $\blieH$, $\lieG$, $\lieH$ etc denote the Lie algebras. By $X^{ss}$, we denote the subset of semisimple elements in $X$. 

Let $\irrG$ be the set of smooth irreducible representations of $\G$. For $(\pi,V_\pi)\in\irrG$, let $\dth(\pi)$ denote the depth of $\pi$. Let $\Theta_\pi$ denote its character.

Let $W_F$ be the Weil group with inertia subgroup $I_F$ and norm $||\ ||$. Let $W_F'=W_F\ltimes\bbC$ be the Weil-Deligne group, where $w\cdot z=||w||z$ for $w\in W_F$ and $z\in\bbC$.
\end{numbering}
\begin{comment}
{\tiny 
\begin{defn}\rm
Let $\gss\in\lieG^{ss}$ be a semisimple element. Let $G'=C_G(\gss)$. Let $\orb(\gss)$ (resp. $\orb'(\gss)$) be the set of $G$-orbits (resp. $G'$-orbits) in $\lieG$ (resp. $\lieG'$)which contain $\gss$ in their closure. Note that there is one-to-one correspondence between $\orb'(\gss)$ and the set of nilpotent orbits $\orb'(0)$ in $\lieG'$.
\end{defn}

\begin{defn}\rm
\begin{enumerate}
\item
Let $\gss\in\lieG^{ss}$. Let $\eta$ be an exponentiable neighborhood of $0$. For $(\pi,V_\pi)\in\irrG$, we say that $\pi$ {\it is $\gss$-asymptotic on $\eta$} if the following holds for any $f\in\Ccs(\eta)$:
\[
\Theta_\pi(f\circ\exp)=\sum_{\orb\in\orb(\gss)}c_\orb\widehat\mu_\orb(f)
\]
for some $c_\orb\in\bbC$, $\orb\in\orb(\gss)$.
\item
{\color{blue} define endoscopic wavefront set}
\end{enumerate}
\end{defn}

\begin{remarks}\rm\ Suppose $\dth(\pi)$ is sufficiently large.
\begin{enumerate}
\item Any $(\pi,V_\pi)\in\irrG$ is $0$-asymptotic on $\lieG_{\dth(\pi)^+}$.
\item Under some assumptions on $F$, for any $(\pi,V_\pi)\in\irrG$, there is $\gss\in\lieG^{ss}$ such that $\pi$ is $\gss$-asymptotic on $\lieG_{\left({\dth(\pi)}/2\right)^+}$.
\item In (2), let $\G'=C_{\G}(\gss)$. Let $\nil'$ be the set of nilpotent elements in $\lieG'$. 
\end{enumerate}
\end{remarks}

\subsection
{\bf Twisted Levi subgroup $\G'$ and $^L\!{\G'}$}

\begin{numbering}\rm 
Let $\bG'$ be an $E$-twisted Levi subgroup of $\bG$ where $E$ is a finite extension of $F$, that is,  $\bG'\otimes E$ is a $E$-Levi subgroup of $\bG\otimes E$. If $E$ is tamely ramified over $F$, we say that $\G'$ is a tame twisted Levi subgroup.
\end{numbering}

\begin{lemma}\rm [Kaletha-regular, Lemma 5.2.8]
Let $\rM\subset\G$ be a tame twisted Levi subgroup. Let $\wM\rightarrow\wG$ be the natural inclusion of dual groups, well defined up to $\wG$-conjugacy. There exists an extension of $\wM\rightarrow\wG$ to a tame $L$-embedding $\LdualM\rightarrow\LdualG$.
\end{lemma}


\proof Let Fix a $\Gal(k)$-invariant pinning $(\wT,\wtB,\{X_{\walpha}\})$ of $\wG$. The unique standard Levi subgroup of $\wG$ dual to the Levi subgroup $M\times\overline k$ of $\G\times\overline k$ is a dual group o f $\rM$, so we can take it as $\wM$. The natural inclusion $\wM\rightarrow\wG$ lies in the canonical $\wG$-conjugacy class.

We have an action of $\Gal(k)$ on $\wG$ coming from the fact that $\wG$ is the dual group of $\G$. We also have an action of $\Gal(k)$ on $\wM$, preserving the pinning of $\wM$ induced by the fixed pinning of $\wG$, coming from viewing $\wM$ as the dual group of $\rM$. The inclusion $\wM\rightarrow\wG$ need not be equivariant for these actions, and in fact the $\Gal(k)$-actoin on $\wG$
}

\

Notion of Endoscopic wave front set, $\gamma$ asymptotic,
Galois structure on twisted Levi/endoscopic subgroups

Types for $GL_n$

$\Gamma$-expansion for $GL_n$ (apres Fiona)

Langlands parameter (Henniart, BZ classification)

Howe's parameterization

Put them together

\end{comment}



